Twisted Riemann bilinear relations and Feynman integrals

Using the framework of twisted cohomology, we study twisted Riemann bilinear relations (TRBRs) satisfied by multi-loop Feynman integrals and their cuts in dimensional regularisation. After showing how to associate to a given family of Feynman integrals a period matrix whose entries are cuts, we investigate the TRBRs satisfied by this period matrix, its dual and the intersection matrices for twisted cycles and co-cycles. For maximal cuts, the non-relative framework is applicable, and the period matrix and its dual are related in a simple manner. We then find that the TRBRs give rise to quadratic relations that generalise quadratic relations that have previously appeared in the literature. However, we find that the TRBRs do not allow us to obtain quadratic relations for non-maximal cuts or completely uncut Feynman integrals. This can be traced back to the fact that the TRBRs are not quadratic in the period matrix, but separately linear in the period matrix and its dual, and the two are not simply related in the case of a relative cohomology theory, which is required for non-maximal cuts.

==> Old_Saves/OldSecTwist.tex <==
%Need to write nicer intro along the lines of this later.

Feynman integrals and their cuts generally involve integrals with multi-valued integrands when considered in dimensional regularization. Consequently, the quadratic relations we want to find and understand will be between integrals of the form 
\begin{align}
\label{gen_twisted_inegral}
    \int_{\Gamma} \Phi \varphi\, , 
\end{align}
where $\Phi$ is a multi-valued function and  $\varphi$ is a rational $n$-form on $X=\mathbb{C}^n-\Sigma$. The space $\Sigma$ includes all hyperplanes, where $\Phi\varphi$ is singular. $\Gamma$ is a closed contour on $X$, i.e. its boundary vanishes. For the integral to be well-defined, a branch choice must be made for $\Phi$. This must be taking into account when taking the boundary of $\Gamma$, as explained below (\ref{homgroup}). Generally, the multi-valued function takes the form
\begin{align}
\label{twist32}
     \Phi= \prod_{i=0}^{r} L_i(\bs{z})^{\alpha_i} 
\end{align}
where  the $L_i(\bs{z})$ are polynomials in the variables $\bs{z}$ and $\alpha_i\in\mathbb{C}$ in the most general case. 
  If $\Phi \varphi$ has branch cuts but no poles the natural framework for these integrals is \textit{twisted (co-)homology}, where the \textit{twist} is the multi-valued function $\Phi$.  We review relevant aspects of twisted (co)-homology in \ref{subsec:twisted}. In many cases, the cuts we consider have additional poles that are not regulated by the twist. In that case, \textit{relative twisted (co-)homology} is the natural framework and we review it in \ref{subsec:reltwist}. Additionally, we comment on limits between the non-relative and relative versions of twisted cohomology. In the final part of this section, we introduce the so-called Riemann bilinear relations \ref{subsec:Riemannbil}.


 We focus here on the basics necessary for the quadratic relations. For a more in depth review of twisted (co-)homology and its application we refer to the literature \cite{yoshida_hypergeometric_1997,aomoto_theory_2011,Mizera:2017rqa,Mizera:2019gea,Mizera:2019ose} and \cite{matsumoto_relative_2019-1,Caron-Huot:2021iev,Caron-Huot:2021xqj} for relative twisted cohomology.

\subsection{Twisted (co-)homology}
\label{subsec:twisted}
In this section, we restrict the twist of (\ref{twist32}) by the condition
\begin{align}
\label{restrict}
\alpha_i\notin \mathbb{Z}\text{ and } \sum_{i=0}^{r} \alpha_i \notin \mathbb{Z}\, .
\end{align}
In this case, $\Phi\varphi$ is a single-valued, holomorphic form on the space  $X= \mathbb{C}^{n}-\Sigma$, where $\Sigma$ denotes the hypersurface on which any of the polynomials $L_i(\bs{z})$ that appear with a non-integer exponent in the twist vanishes or diverges, including the hypersurfaces at infinity. We call these the \textit{regulated boundaries}. In the context of Feynman integrals, the choice of a twist (i.e. the Baikov polynomials) fixes an integral family and by using integration by parts (IBP) identities , we can find a basis for this family. Similarly, in the framework of twisted cohomology, the twist defines a family of differentials and a connection which accounts for the mulitvaluedness of the integrals
\begin{align}
\label{connect}
\nabla = \rd +\Omega \wedge \cdot \text{ with } \Omega = \frac{\rd \Phi}{\Phi} =\rd \log \Phi\, \, . 
\end{align}Working modulo exact forms -- i.e. $\varphi \sim \varphi +\nabla \tilde{\varphi}$ --means working modulo forms that vanish upon integration.  This is equivalent to the approach of working with IBP identities in the context of Feynman integrals.  In that sense we 
only consider elements of the \textit{twisted cohomology group} 
\begin{align}
\label{twistedcoh}
    H_{\text{dR}}^k (X, \nabla)&=C^k(X,\nabla)/B^k(X,\nabla) \text{ with } \\
    C^k(X,\nabla)&=\{ k-\text{forms }\varphi \text{ on } X\, |\, \nabla \varphi = 0 \} \text{ and }\\
    B^k(X,\nabla)&= \{ k-\text{forms }\nabla\varphi\, |\, \varphi \text{ a $k-1$-form}\} \, . 
\end{align}
Note, that only the middle cohomology is nonzero in the twisted case, which is why we only need $k=n$ throughout this paper. The elements of $H_{\text{dR}}^{n}(X,\nabla)$ are the \textit{twisted co-cycles} and they have a finite basis. The contours we consider are \textit{twisted cycles} $\gamma \otimes \Phi_\gamma$ from 
\begin{align}
\label{homgroup}
    C_k(X,\check{\mathcal{L}}) =  \{k-\text{cycles }\gamma \otimes \Phi|_{\gamma}\,  |\, \partial (\gamma\otimes \Phi|_{\gamma} )=0\} \, . 
\end{align}
By the notation $\gamma \otimes \Phi|_\gamma$ we indicate, that we assign a branch of $\Phi$ to $\gamma$.  This branch choice is specified by the locally constant sheaf $\check{\mathcal{L}}$ generated by $\Phi$.  The operation $\partial (\gamma\otimes\Phi|_{\gamma})$ maps the contour to its boundary and restricts the branch to this boundary. We denote the boundaries by $B_k(X,\check{\mathcal{L}})= \{k-\text{cycles }\partial \left(\gamma\otimes \Phi|_{\gamma}\right)\}$. As integration contours, we want to consider only closed contours on $X$ modulo boundaries, i.e. elements of the \textit{twisted homology group}:
\begin{align}
\label{twistedho}
H_k(X, \check{\mathcal{L}}) =C_k(X,\check{\mathcal{L}})/ B_k(X,\check{\mathcal{L}}) \, . 
\end{align}Generally for the cases considered here, the cycles are regularized chambers between multi-valued boundaries. The regularization scheme is explained in \cite{yoshida_hypergeometric_1997,kita_intersection_1994-2,aomoto_theory_2011, Bhardwaj:2023vvm, Duhr:2023bku}.  We obtain integrals such as (\ref{gen_twisted_inegral})  by pairing elements of the twisted homology and cohomology group via the \textit{period pairing}: 
\begin{align}
 \langle \gamma |\varphi]= \int_{\gamma} \Phi \varphi\, . 
\end{align}
Acting with this pairing on the basis elements $\gamma_i$ of $H_k(X,\check{\mathcal{L}})$ and $\varphi_j$ of $H_{\text{dR}}^k(X,\nabla)$, we obtain the period matrix $\bs{P}$ with entries
\begin{align}
 P_{ij}= \langle\varphi_i| \gamma_j]\  =\int_{\gamma_j}\Phi\varphi_i\, . 
\end{align}
By replacing the twist with its inverse in (\ref{connect}) one defines the dual connection $\check{\nabla}=\rd -\rd \log \Phi \wedge $ and obtains similar to 
(\ref{twistedcoh}) and (\ref{twistedho})  the corresponding dual twisted (co-)homology groups:
\begin{align}
H_{\text{dR},c}^k \left(X, \check{\nabla}\right) &= \{ \text{compactly supported } k-\text{forms } \check{\varphi} \, |\, \check{\nabla} \check{\varphi}_c =0\}/ \{\text{exact forms}\}\\
H_k^{\text{lf}}(X,\mathcal{L}) &=  \{\check{\gamma} \otimes \Phi^{-1}|_{\check\gamma} \text{ locally finite} \, |\,  \partial \check{\gamma}  =0\} / \{ \text{boundaries }\partial\tilde{\check{\gamma} }\} \, .
\end{align}
The restriction to compactly supported forms for the dual cohomology group is necessary for the intersection pairing between twisted co-cycles, 
\begin{align}
    \langle \varphi_A|\check\varphi_{B,c}\rangle&=\int_X \varphi_A\wedge \check\varphi_{B,c}
\end{align}
to be well-defined. For a given form $\varphi$ one can compute a compactly supported version with the methods described  in \cite{Mizera:2017rqa,Mastrolia:2018uzb} and we denote this compactly supported version by $\left[\varphi\right]_c$. The intersection matrix $\bs{C}$ has entries
\begin{align}
    C_{ij} = \frac{1}{(2\pi i)^k} \langle \varphi_i |\check{\varphi}_j\rangle \, . 
\end{align}
The intersection pairing for the twisted homology group and its dual, $
[\check{\gamma}_A|\gamma_B]$ counts the intersections of the two contours, taking into account their orientations as well as the branch choice for $\Phi$ and $\Phi^{-1}$ loaded onto them. More details on their computation can be found in \cite{yoshida_hypergeometric_1997, Duhr:2023bku,kita_intersection_1994-2}. We denote by $\bs{H}$ the intersection matrix  with entries 
\begin{align}
    H_{ij}=[\check{\gamma}_j|\gamma_i]\, . 
\end{align}
Since the non-dual twisted cycles are already regularized, the  dual cycles are only required to be locally finite for the intersection pairings of $\bs{H}$ to be well-defined, i.e. they can be chosen as line segments without the regularization required for the cycles. Pairing the basis elements of both dual  groups, one obtains the dual period matrix $\check{\bs{P}}$ with entries
\begin{align}
    \check{P}_{ij} = [\check{\gamma}_j|\check{\varphi}_i\rangle = \int_{\check{\gamma}_j} \Phi^{-1} \check{\varphi}_i\, .  
\end{align}
Now, we want to stress a property of twisted cohomology with only regulated boundaries, that will be important for us when considering the period matrix as a matrix of cuts of Feynman integrals. For standard  twisted cohomology with the restriction of (\ref{restrict}), we can choose as a basis of the dual twisted cohomology group the compactly supported version of the basis of the twisted cohomlogy group and upon integration, these do not differ. Thus, the difference between the period matrix and its dual lies only in the choice of the twist: 
\begin{align}
    \Phi^{-1}=\left(\prod_{i=0}^r L_i(\bs{z})^{\alpha_i} \right)^{-1}=\prod_{i=0}^r L_i(\bs{z})^{-\alpha_i} \, . 
\end{align}
More explicitely, in that case we obtain:
\begin{align} 
\check{P}_{ij}=\int_{\check{\gamma}_j} \Phi^{-1} \check{\varphi}_i = \int_{\check{\gamma}_j} \prod_{i=0}^r L_i(\bs{z})^{-\alpha_i}{\varphi}_i= P_{ij}|_{\alpha_k\rightarrow -\alpha_k}\, . 
\end{align}
If all $\alpha_i$ are proportional to $\varepsilon$, that means 
\begin{align}
    \bs{\check{P}}(\varepsilon)=\bs{P}(-\varepsilon)\, . 
\end{align}
Note, that this implies that one can write the dual period matrix in terms of the period matrix with flipped parameters $\alpha_i$ or $\varepsilon$. 


\begin{example}[Gauss hypergeometric ${}_2F_1$ function]
\label{example11}

We consider Gauss hypergeometric function 
\begin{align}
\label{eq_f21}
    {}_2F_1(a,b,c;x)=\frac{\Gamma(c)}{\Gamma(b)\Gamma(c-b)} \int_0^1 z^{a-1} (1-z)^{c-a-1} (1-xz)^{-b}\rd z\, .
\end{align} 
as a simple example. These integrals can be interpreted as periods of a twisted cohomology with the twist defined by the product in the integrand. For the examples discussed here, we choose 
\begin{align}
\label{eq_twistF21}
    \Phi = z^{ \alpha_0 } (1-z)^{\alpha_1} \left(1-x^{-1}{z}\right)^{\alpha_{x}} \, 
\end{align}
with $0<\alpha_i<1$ a non-integer parameter. In this case, $X=\mathbb{C}-\{0,1,x, \infty\}$. We choose for the basis of forms in $H_{\text{dR}}^1(X,\nabla)$
\begin{align}
\label{herenotchange}
\varphi_1=-  \frac{C_{N}\rd z}{z} \text{ and } \varphi_2=\frac{(1-x)\rd z}{(1-z)\left(z-x\right)}  \text{ with } C_{N}=\sqrt{\frac{\alpha_0 (\alpha_0+\alpha_1)}{\alpha_1} }
\end{align}
and for the dual basis
\begin{align}
\check{\varphi}_1=- \left[ \frac{C_{N}\rd z}{z}\right]_c \text{ and } \check{\varphi}_2=\left[\frac{(1-x)\rd z}{(1-z)\left(z-x\right)}\right]_c  
\end{align}
For the basis of contours in $H_1(X,\check{\mathcal{L}})$ we choose the regularized versions of the dual basis elements $\check{\gamma}_1=[0,1] \text{ and } \check{\gamma}_2=[x,\infty]$.
%\begin{align}
%\check{\gamma}_1=[0,1] \text{ and } \check{\gamma}_2=[x,\infty]\, 
%\text{ and }\gamma_1=[0,1]_\text{reg}\,,\quad\gamma_2=[x,\infty]_\text{reg}. 
%\end{align}
Then, the period matrix $\bs{P}$ has the entries 
\begin{align}
\label{firstperiod}
P_{11} &= - C_{N} \frac{\Gamma(\alpha_0  ) \Gamma(\alpha_1 +1)}{\Gamma(\alpha_{01}   +1)} {}_2F_1(\alpha_0 , -\alpha_{x}  , \alpha_{01} +1; 1/x)\,  ,\\
P_{12} &=C_{N} e^{i\pi \left(\alpha_{1x}  +1\right)} x^{\alpha_{01} } \frac{\Gamma(\alpha_{x}   +1 ) \Gamma(-\alpha_{01x}   )}{\Gamma(1-\alpha_{01} )} {}_2F_1(-\alpha_1 , -\alpha_{01x} , -\alpha_{01}  +1; 1/x) \\
P_{21}&= \left(1-x^{-1}\right)\frac{\Gamma(\alpha_0 +1)\Gamma(\alpha_1 )}{\Gamma(\alpha_{01} +1)} {}_2F_1(\alpha_0  +1, 1-\alpha_{x}  , \alpha_{01} +1;1/x)\\
P_{22} &= \left(1-x^{-1}\right)e^{i\pi \left(a_{1x} -2\right)} x^{\alpha_{01} } \frac{\Gamma(a_{x} )\Gamma(-\alpha_{01x} +1)}{\Gamma(-\alpha_{01} 
+1)}{}_2F_1\left(1-\alpha_1 , -\alpha_{01x} +1,-\alpha_{01} +1,1/x\right)
\end{align}  where we use the notation $\alpha_{ij\dots} = \alpha_i+\alpha_j+\dots$. The dual period matrix can be obtained as 
\begin{align}
    \check{\bs{P}}=\bs{P}|_{\alpha_i\rightarrow -\alpha_i}\, . 
\end{align} 
Note, that the replacement $\alpha_i\rightarrow-\alpha_i$ does \textit{not} apply to the $\alpha_i$ of $C_N$, but $C_N$ is a constant appearing in both the period matrix and its dual. The intersection matrices are 
\begin{align}
\label{cmat}
\bs{C}&=\begin{pmatrix} -\frac{ \alpha_{01}\alpha_{1x}}{\alpha_1\alpha_{01x} } & 0 \\ 0&-\frac{\alpha_{1x}}{\alpha_1\alpha_x  }
    \end{pmatrix} \\
\label{hmatin}
    \bs{H}&=\begin{pmatrix}
        -\frac{i}{2} \left(\cot(\pi \alpha_0 )+\cot(\pi \alpha_1 )\right) &0 \\ 0 & -\frac{i}{2} \csc(\pi \alpha_x )\sin(\pi \alpha_{01}  ) \csc(\pi \alpha_{01x} )
    \end{pmatrix}\, . 
\end{align}
\fpnote{Want to think about the signs here again in the end.}
\end{example}

\subsection{Twisted relative (co-)homology}
\label{subsec:reltwist}
As detailed in \cite{Caron-Huot:2021iev,Caron-Huot:2021xqj}, duals of Feynman integrands live in a \textit{relative twisted cohomology} group. In this framework, we can relax the restrictions on the twist in  (\ref{restrict}) and allow $\alpha_i \in \mathbb{Z}$ or equivalently, treat integrands $\Phi \varphi$ with poles that are not regulated by $\Phi$ so that boundary terms might arise. The basic idea of this framework is that cycles of a relative twisted homology group have no boundaries at unregulated points, so that poles of the cocycles do not cause any problems.
Equivalently, we allow the dual cycles to have boundaries in a subcomplex  consisting of the unregulated boundaries and in turn the relative \textit{dual} co-cylces have additional terms  that keep track of boundary contributions. We give a very brief review here, for more details on this framework see \cite{matsumoto_relative_2019-1,Caron-Huot:2021xqj, Caron-Huot:2021iev} and for its applications in physics see \cite{Giroux:2022wav,De:2023xue,Bhardwaj:2023vvm,Brunello:2023rpq}.

For the remainder of this section, we define the following sets of hyperplanes:
\begin{align}
    \Sigma &=\{\bs{z}\, |\, L_i(\bs{z}) = 0 \wedge \alpha_i \notin\mathbb{Z}\} \cup \{\infty\} \\
    D_+&=\{ \bs{z}\, |\, \Phi\varphi(\bs{z}) = 0\} \\
    D_- &= \{\bs{z}\, |\, \bs{z} \text{ is a pole of }\Phi\varphi(\bs{z})\wedge  \bs{z} \notin \Sigma\} \, . 
\end{align}
Additionally, we denote:
\begin{align}
    X_+&= \mathbb{C}^n- \Sigma -D_+\\
    X_-&=\mathbb{C}^n -\Sigma -D_-\, . 
\end{align}

\paragraph{Relative twisted homology}
Since the forms we consider vanish on $D_+$, we can allow for cycles with boundaries on $D_+$ in our definition of a closed cycle. In that sense, we define \textit{relative twisted cycles} as 
\begin{align}
\label{relativecycels}
    C_k(X_-,D_+,\check{\mathcal{L}}) = C_k(X_-,\check{\mathcal{L}})/C_k(D_+,\check{\mathcal{L}}) \, , \text{ with }  C_k(D_+,\check{\mathcal{L}})=C_k(X_-,\check{\mathcal{L}}) |_{D_+}\, . 
\end{align}
Based on this, we can define the \textit{relative twisted homology group}:
\begin{align}
    H_k(X_-,D_+,\check{\mathcal{L}}) =  C_k(X_-,D_+,\check{\mathcal{L}})/  B_k(X_-,D_+,\check{\mathcal{L}})\, .
\end{align}
As a basis for the homology group $H_k(X_-,D_+,\check{\mathcal{L}})$ we generally choose a combination of spheres around the hypersurfaces in $D_+$ and (regulated) chambers between the hypersurfaces $\{L_i(\bs{z})=0\}$ in $\Sigma$ . We provide an example in (\ref{eq_reltwist}). Since the role of zeroes and poles is reversed in the dual\footnote{Note, that we can always define any single-valued factors of the form $\varphi$ with poles or zeroes to be part of the twist (with an integer exponent). In that sense the notion of reversing the poles and zeroes when taking the inverse of the twist is well-defined.}, where $\check{\Phi}= \Phi^{-1}$, the dual relative twisted homology group is 
\begin{align}
H_k(X_+, D_-,\mathcal{L}) = C_k(X_+,D_-,\mathcal{L})/ B_k(X_+,D_-,\mathcal{L}) \, . 
\end{align}
%\csnote{found the notation for the spaces $X$ a bit confusing here but we should either stick to denoting by $\check{X}$ the space with only the regulated boundaries taken out or the other way round, I think which way we define it doesnt matter, but I changed everything now so that it aligns with andrzejs definitions}, since poles of the twist become zeroes of the inverse twist.   

\paragraph{Relative twisted cohomology}
Similarly, one defines the relative twisted cohomology group
\begin{align}
\label{relativetwistedcohojmology}
    H^k_{\text{dR}} = C^k(X_-,D_+, \nabla)/ B^k(X_-,D_+,\nabla) \, ,
\end{align}
where the relative twisted co-cycles are defined by $ C^k(X_-,D_+, \nabla)= C^k(X_-,\nabla)/C^k(D_+, \nabla)$. Note, that for cases, where $\Phi\varphi$ has no zeroes that are not regulated by the twist: 
\begin{align}
    H_{\text{dR}}^k (X_-,D_+,\nabla)\cong H_{\text{dR}}^k (X_-,\nabla)\, . 
\end{align}
This applies to all examples for cuts of Feynman integrals that we consider here. One needs to be more careful when considering the dual relative twisted cohomology group 
\begin{align}
    H^k_{\text{dR}}(X_+,D_-,\check{\nabla}) = C^k(X_+,D_-,\check{\nabla})/B^k(X_+,D_-,\check{\nabla}) \, . 
\end{align}
and more importantly, its compactified version $H^k_{\text{dR}}(X_+,D_-,\check{\nabla})$ that is necessary for a well defined intersection pairing. Forms of $H^k_{\text{dR}}(X_+,D_-,\check{\nabla})$  generally have the form  
%Similarly, \textit{relative twisted co-cycles} are elements of 
%\begin{align}
%    C^k (\check{X}, D, \nabla) = C^k (\check{X},\nabla) / %C^k(D,\nabla) \text{ with } C^k (D,\nabla) = %C^k(\check{X},\nabla)|_D
%\end{align}
%and a \textit{relative twisted cohomology group} is defined as 
%\begin{align}
%    H^{k}_{\text{dR}} (\check{X},D,\nabla)= %C^k(\check{X},D,\nabla)/ B^k(\check{X},D,\nabla)\, . 
%\end{align}
%A basis choice for the non-dual cocycles translates directly from the non-relative case, since the non-dual cycles do not have unregulated boundaries and hence are element of $ H^{k}_{\text{dR}} (X,\nabla)$. \fpnote{@Cathrin I would be very in favor of changing this back to the previous version. Just because the non-dual side is the same as in the non-relative case does not mean that one should replace it. I am also not sure if taking the relative on one side and the non-relative on the other is actually mathematically sound and works with the limits we are discussing. We can avoid saying something wrong regarding these subtleties by just sticking to one framework without having any additional problems due to that. Mixing frameworks might also be unnecessarily confusing.} \csnote{I think we understand this a bit differently, the way i understand this, only dual forms are elements of a relative cohomology group. the non-dual side is just the same, there is no mixing frameworks? saying relative non-dual cohomology makes no sence to me because there is just one relative group, namely the one we choose the dual elements of. the \textit{relative framework} refers only to the dual cohomology side/non-dual homology side beeing relative. Maybe i understand this really wrong, but i guess we should talk about this tomorrow. If you are really sure, change it back}\fpnote{I am quite sure that the way you phrased it now is wrong. The dual relative twisted cohomology must be a well defined dual of something and that something is the relative twisted cohomology. Formally, it can't be the dual of a non-relative twisted cohomology (even thouhg it might practically be), because that dual is already a non-relative dual cohomology. This is also the way it is introduced in \cite{matsumoto_relative_2019-1}. Andzrej just doesn't care about that side much and it is the same as the non-relative case anyways so it doesn't matter. But mathematically, it does not make sense to say there is a dual relative twisted cohomlogy but not a twisted relative cohomology. But let's talk about this tomorrow.}\csnote{doesnt dual space just mean that it is the space of linear functionals of the space to some underlying field? I dont really understand what the problem is as long as the intersection pairing/bilinear mapping is well defined, which is the case because we know about the isomorphism of the relative group to the compactly supported versions. But i will look into the matsumoto paper again till tomorrow, maybe i understand it better then}\fpnote{I believe you that this is true. but if we do it this way, we would need to write/justify all these things for it to be formally correct. This would mean writing a whole paragraph about some subtleties that are not relevant for the paper instead of just saying "relative twisted cohomology looks like the non-relative one" and refering to the matsumoto paper where he probably worked it all out.} In contrast, \textit{dual twisted co-cycles} are elements of $H_{\text{dR},c}^k(\check{X},D,\check{\nabla})$. Practically, this is realized via the $\delta$-symbols of \cite{Caron-Huot:2021iev,Caron-Huot:2021xqj} where a general relative co-cycle $\check{\varphi} \in H_{\text{dR},c}^k(\check{X},D,\check{\nabla})$ is of the form: 
\begin{align}
    \check{\varphi} = \theta \psi + \delta_1(\theta \psi_1)+\dots + \delta_{1,2} \left(\theta \psi_{1,1}\right)+ \dots \, .
\end{align}
Here $\theta$ is a symbol that keeps track of possible boundary terms and the sum is over all (intersections of) sub-boundaries of $D_-$. The form $\delta_{i_1,\dots,i_n}({\phi}_{i_1,\dots,i_n})$ is the \textit{Leray coboundary} of a form ${\phi}|_{i_1,\dots,i_n}$  living on the boundary $\{D_{i_1}=0\}\cup \dots \cup\{ D_{i_n}=0\}$. In practice, these Leray coboundaries can be represented explicitly by 
\begin{align}
\delta_{i_1,\dots,i_n}({\phi}_{i_1,\dots,i_n})=\frac{\Phi}{\Phi|_{i_1,\dots,i_n}} \rd\theta_{i_1}\wedge\dots \rd\theta_{i_n} \wedge {\phi}_{i_1,\dots,i_n}
\end{align}
where for simplicity we treat $\rd\theta$ as the Heaviside function. Details on the construction and meaning of $\rd \theta$ can be found in \cite{Caron-Huot:2021iev,Caron-Huot:2021xqj,Giroux:2022wav}. For one-forms, this translates to the statement that a dual basis of $H^1_{\text{dR}}(X_+,D_-,\check{\nabla})$ can be built from forms
\begin{align}
\label{zibasis}
\delta_{z_i}(1)=\frac{\Psi}{\Psi|_{z_i}} \rd\theta(z-z_i) \text{ for } z_i \text{ a pole}
\end{align}
and compactifications of twisted co-cycles ${\phi}_{\text{reg}}$  with regulated singularities 
\begin{align}
\left[\phi_\text{reg}\right]_c=\phi_\text{reg} \prod_i \theta(z-z_i) +\sum_i\psi_i \rd \theta(z-z_i)
\end{align}
with ${\phi}_{\text{reg}}$ chosen as in the non-relative case.
The functions $\psi_i$ are the local primitives defined by the twist as
$\check{\nabla}\psi_i =\phi_{\text{reg}}$. With this basis choice, the intersections can be computed with residues:
\begin{align} 
\langle \varphi|\delta_{1,\dots,n}(\check{\phi})\rangle&=\text{Res}_{1,\dots,n}\left(\frac{\Phi}{\Phi|_{i_1,\dots,i_n}}\varphi\right)\,,\\
\langle\varphi|\left[\phi_\text{reg}\right]_c\rangle&=\sum_k \text{Res}_{z=z_k}(\psi_k \varphi)\, ,
\end{align}
respectively. \fpnote{@Cathrin: Es gibt in (3.47) links ein $\phi$, aber nicht rechts. Ist das richtig so?}\csnote{jo, das steckt in der local primitive}

\begin{example}[Gauss hypergeometric ${}_2F_1$ function in relative twisted cohomology]
\label{example21}

We take again the ${}_2F_1$ function with the twist of (\ref{eq_twistF21}) as an example. But now, we consider the case with a pole at $x$ by taking $\alpha_x\rightarrow 0$, such that the twist is given by
\begin{align}
\label{eq_reltwist}
    \Phi= z^{\alpha_0 }(1-z)^{\alpha_1 }\left(1-x^{-1}z\right)^{0}\, . 
\end{align}
For the basis forms we choose  
\begin{align}
\label{eq_relabasis}
    \varphi^{\text{rel}}_1= -C_{N}  \frac{\rd z}{z} \text{ and } \varphi^{\text{rel}}_2 = \frac{\rd z (1-x)}{(z-x)(1-z)}\, ,\\
\check{\varphi}^{\text{rel}}_1=-C_{N}\left[\frac{\rd z}{z}\right]_c\text{ and } \check{\varphi}^{\text{rel}}_2=\delta_x(1)= \Phi \left(\Phi|_{z\rightarrow x}\right)^{-1} \rd \theta(z-x)\, . 
\end{align}
For the contours, we choose $\gamma_1$ to be the loaded cycle supported on the regularized interval $[0,1]$ and $\gamma_2$ to be the normalised $\varepsilon$-circle $(2\pi i)^{-1}S_\varepsilon(x)$. This second cycle differs from the choice we made for the non-relative case, where all basis cycles are regularized intervals. This is, because the function $\Phi$ is not multi-valued at $x$ and thus, the circle around it is already a closed contour. For the dual cycles we choose as a basis the loaded cycles supported on the intervals $[0,1]$ and $[x,\infty]$. 
In this case, the period matrix is given by 
\begin{align}
    \label{pmatrel}
P_{11}&= - C_{N}  \frac{\Gamma(\alpha_0 )\Gamma(\alpha_1 +1)}{\Gamma(\alpha_{01} +1)} \\
P_{12}&= 0\\
P_{21}&=-\frac{1-x}{x} \frac{\Gamma(\alpha_0+1)\Gamma(\alpha_1 )}{\Gamma(\alpha_{01} +1)}{}_2F_1\left(\alpha_0 +1,1,\alpha_{01} +1,\frac{1}{x}\right)\\
P_{22}&= x^{\alpha_0 } (1-x)^{\alpha_1 } \, 
\end{align}
and the dual period matrix by
\begin{align}
\label{pmatreldual}
\check{P}^{\text{rel}}_{11}&=-C_{N}  \frac{\Gamma(-\alpha_0 )\Gamma(-\alpha_1 +1)}{\Gamma(-\alpha_{01} +1)}\\
\check{P}^{\text{rel}}_{12}&=-C_{N}e^{-\pi i \alpha_1 }   \,  x^{-\alpha_{01} } \frac{\Gamma(\alpha_{01} )}{\Gamma(\alpha_{01} +1)} {}_2F_1\left(\alpha_{01} , \alpha_1 , \alpha_{01} +1,\frac{1}{x}\right) \\
\check{P}^{\text{rel}}_{21} &= 0\\
\check{P}^{\text{rel}}_{22} &= x^{-\alpha_0 } (1-x)^{-\alpha_1 } \, . 
\end{align}
The intersection matrices for $x>1$ are
\begin{align}
\label{intersectionsrelative}
  \bs{H}^{\text{rel}}=\begin{pmatrix}
     -\frac{i}{2}\left(\cot\left(\pi  \alpha_0\right)+\cot\left(\pi  \alpha_1\right)\right)&0\\ 0 & -\frac{1}{2\pi i}
    \end{pmatrix}  \text{ and } \bs{C}^{\text{rel}}=\begin{pmatrix}
     -1&0\\ 0 & 1
    \end{pmatrix} \, . 
\end{align}
\end{example}

\subsection{The Riemann bilinear relations in different frameworks}
\label{subsec:Riemannbil}
In (relative) twisted cohomology there  are the \textit{completeness relations} 
\begin{align}
1&=(2 \pi i)^{-n} \ket{\check{\varphi}_i} (C^{-1})_{ij} \bra{\varphi_i}\,,\\
1&=|\gamma_i](H^{-1})_{ji}[\check{\gamma}_j|\,.
\end{align}
Those relations combined yield the \textit{Riemann bilinear relations}  
\begin{align}
\label{generalriemann}
    C= \frac{1}{(2\pi i)^n} P \left(H^{-1}\right)^T \check{P}^T \Leftrightarrow 
    H= \frac{1}{(2\pi i)^n} P^T \left(C^{-1}\right)^T \check{P}\, . 
\end{align} 
 As explained in \ref{subsec:twisted}, for standard twisted cohomology (with only non-integer exponents in the twist), one can choose bases for the twisted cohomology group and its dual so that the period matrix and the dual period matrix only differ by $\bs{\alpha} \rightarrow -\bs{\alpha}$. Then the Rieman bilinears specialize to relations that are quadratic in the periods
\begin{align}
\label{epminepRiemannn}
    C= \frac{1}{2\pi i} P \left(H^{-1}\right)^T \left({P}|_{\alpha_i\rightarrow -\alpha_i}\right)^T \Leftrightarrow 
    H= \frac{1}{2\pi i} P^T \left(C^{-1}\right)^T \left({P}|_{\alpha_i\rightarrow -\alpha_i}\right)\, .
\end{align}
This form is particularly useful, when the period matrix is constructed from objects of interest (e.g. cuts of Feynman integrals) and we want the same to be true for the dual period matrix. Due to the necessity of relative dual forms such as (\ref{zibasis}), this is generally not possible in the framework of relative twisted cohomology. We illustrate this with an example. 

\begin{example}[Riemann  bilinear relations for the  Gauss hypergeometric ${}_2F_1$ function]
We give examples for the twisted Riemann bilinear relations obtained from the period and intersection matrices of the examples \ref{example11} and \ref{example21}. 

\noindent \textbf{Relations in the non-relative framework} 
In the non-relative example \ref{example11}, we obtain relations for the hypergeometric ${}_2F_1$ such as 
\begin{align}
    \frac{\pi \alpha_{01}\alpha_{1x}}{\alpha_1\alpha_{01x}} = \frac{P_{11} \left(P_{11}|_{\alpha_i\rightarrow -\alpha_i}\right)}{\cot(\pi\alpha_0)+\cot(\pi\alpha_1)}+ \frac{\sin(\pi\alpha_x)\sin(\pi\alpha_{01x})}{\sin(\pi\alpha_{01})} P_{12} \left(P_{12}|_{\alpha_i\rightarrow -\alpha_i}\right)
\end{align}
where the entries $P$ are the ones of (\ref{firstperiod}) in terms of hypergeometric functions. Thus, we obtain quadratic relations between the periods. 

\noindent \textbf{Relations in the relative framework} 
On the other hand, we consider the relations we obtain for the example of a hypergeometric ${}_2F_1$ function with a twist $\Phi= z^{\varepsilon\alpha_0}(1-z)^{\varepsilon\alpha_1}(1-zx)^0$, i.e. with a pole at $x^{-1}$.  We consider the Riemann bilinear relations in the form $ C= \frac{1}{(2\pi i)^n} P \left(H^{-1}\right)^T \check{P}^T $ with the intersection and period matrices as in (\ref{intersectionsrelative}), (\ref{pmatrel}) and (\ref{pmatreldual}). Most entries of this matrix relation are trivial. In the (2,1) entry, we obtain the relation
\begin{align}
0=&\frac{1-x}{x} \left(i +\cot(\pi \varepsilon\alpha_1)\right){}_2F_1\left(1+\varepsilon\alpha_0,1,1+\varepsilon\alpha_{01},\frac{1}{x}\right) \\
& +(1-x)^{\varepsilon \alpha_1} x^{-\varepsilon\alpha_1} \csc\left(\pi \varepsilon\alpha_1\right) {}_2F_1\left(\varepsilon\alpha_{01},\varepsilon\alpha_1,1+\varepsilon\alpha_{01},\frac{1}{x}\right)\, . 
\end{align}
\end{example}
 We can still express the dual period matrix in terms of the periods by solving the twisted Rieman bilinear relations for $\check{P}$. However, in that way the Rieman bilinears do not yield quadratic relations between the periods beyond the ones on the diagonale. Since we saw, that we obtain quadratic relations in the non-relative framework, but not in the relative one, we now regulate the poles by taking a limit of the non-relative twisted cohomology and consider the relations obtained in this framework. For simplicity, we discuss this for one pole and $n=1$. \fpnote{The discussion now is highly specialized anyways, maybe we should connect discussion and exmaple immediately from here on and say in the end that one can also do this for more general cases.} In this case, we introduce a factor
\begin{align}
\label{eq_regulator}
    (z-\xi)^{\rho}\, . 
\end{align}
 In the generic case, we would introduce such a factor for each pole $\xi_i$ to the twist. The \textit{regulators} ${\rho_i}$ are taken to zero after the computation of the intersection and period matrices. For simplicity, let us assume there is only one such factor with regulator $\rho$. This is the same approach that is employed in \cite{Chestnov:2022alh, Brunello:2023rpq}. A comparison between taking the limit of regulators and working with relative twisted cohomology from the start was discussed in detail in \cite{Brunello:2023rpq}. Ideally, we would hope for the limit of the regulator to preserve the property that $\bs{\check{P}}=\bs{P}|_{\alpha_i\rightarrow -\alpha_i}$ and at the same time the non-degenerance of the intersection matrices. We consider two ways of taking this limit and each of them preserves only one of these properties. On one hand, one can Laurent-expand the entries of the intersection matrix $\bs{C}$ in $\rho$,
 \begin{align}
     C_{ij}= \sum_{i} C_{ij}^k (z-\xi)^k
 \end{align}
 and take the leading order term in each entry separately according to the rule: 
 \begin{align}
 \label{limitlim}
     C_{ij} \rightarrow C_{ij}|_{LT} = \begin{cases} C_{ij}^0&  \check{\varphi}_j\text{ has no pole in } \xi\\
     C_{ij}^{-1}&  \check{\varphi}_j\text{ has a pole in } \xi\, . 
     \end{cases}
 \end{align}
 This is the approach  suggested in \cite{Brunello:2023rpq}.  It can also be reproduced by first rotating the matrix with a transformation matrix that contains functions of the $\rho$, such that no entry has a leading order term of an  order lower than zero and then simply taking the limit $\rho\rightarrow 0$. This rotation corresponds to a change in the dual cohomology basis  and can also be employed to the dual period matrix. A similar approach can be taken for the homology intersection matrix $\bs{H}$, though the transformation matrices involved also change the period matrix and include also functions of the $\alpha_i$.  Having obtained these transformations,  we can take the limit $\rho\rightarrow 0$ on all period and intersection matrices. This approach produces non-degenerate intersection matrices and their corresponding period matrices for some basis in a relative twisted cohomology. But that also means that the dual period matrix is not related to the period matrix through a simple exchange of the $\alpha_i$ and we can not get quadratic relations beyond the diagonale from the twisted Riemann bilinear relations. 
 %the obtained intersection matrix corresponds to an intersection matrix that can be reproduced (for a certain canonical basis) in the relative framework. Taking the limit according to \cite{Brunello:2023rpq} includes rotating the corresponding dual period matrix. Applying this rotation yields exactly the dual period matrix that we get from the canonical relative basis choice so that the resulting Rieman bilinears are equivalent to those obtained in the relative framework. 
 
On the other hand, we can take the limit with respect to an overall leading order without introducing a rotation and indeed the dual period matrix in the limit is still related to the period matrix by $\alpha_i\rightarrow -\alpha_i$.  However, in this case, one obtains degenerate intersection matrices, which means that these are not intersection matrices of a full  basis of the target space but only of a subspace. As a consequence, we obtain only a subset of the relations we obtain in the relative framework. We illustrate this with the example of the ${}_2F_1$ function by comparing the two limit procedures. 

\begin{example}[Riemann  bilinear relations for the  Gauss hypergeometric ${}_2F_1$ function [continued]] 
We consider again the example of \ref{example21}, but this time start with (\ref{eq_twistF21}) and set $\alpha_x=\rho$. Then, we Laurent expand the intersection numbers in $\rho$:
%. According to \cite{Brunello:2023fef}, for intersections stemming from unregulated poles, the intersection number are of the form $C_{ij}\sim (\rho)^{-1}(C_{ij})_\text{LT}+\mathcal{O}(\rho^0)$. Intersections stemming from regulated poles are finite $C_{ij}\sim (C_{ij})_\text{LT}+\mathcal{O}(\rho)$ so that the Laurent expansion of the intersection matrix (\ref{cmat})) is given by 
\begin{align}
\label{355}
\bs{C}(\rho)&=\begin{pmatrix} -1+\mathcal{O}(\rho)&0\\ 0&-\frac{1}{\rho}+\mathcal{O}(\rho^{0})\end{pmatrix}\\
\bs{H}(\rho)&=\begin{pmatrix} -\frac{i}{2}\left(\cot(\pi \varepsilon\alpha_0) +\cot(\pi \alpha_1)\right)+\mathcal{O}(\rho)&0\\ 0&\frac{1}{2i\pi\rho}+\mathcal{O}(\rho^{0})\end{pmatrix} \, . 
\end{align} 
Now we can take the limit of $\rho$ in the two ways described above.

\noindent \textbf{Limit from the non-relative case with the LT approach of \cite{Brunello:2023fef}} \fpnote{I remove the $\varepsilon$ here so that it fits with the examples before. please check if it is still correct that way.} 
%To obtain an invertible intersection matrix in the relative limit we take the leading order term entry-by-entry.
Taking the limit as described in (\ref{limitlim}), we obtain: 
\begin{align}
\label{leadingterm}
    \bs{C}_{\text{LT}} =\begin{pmatrix}
        -{1}  & 0\\ 0&-1
    \end{pmatrix}\text{ and }
    \bs{H}_{\text{LT}}= \begin{pmatrix}
        -\frac{i}{2}\left(\cot(\pi \alpha_0) +\cot(\pi \alpha_1)\right)&0 \\
        0&\frac{1}{2i\pi}
    \end{pmatrix}\, . 
\end{align}
Note, that $\bs{H}_{LT}$ and  $\bs{C}_{LT}$ are the same intersection matrices as those in (\ref{intersectionsrelative}) that were obtained in the relative framework with the basis (\ref{eq_relabasis}). 
%As described in  \cite{Brunello:2023fef}, the canonical relative basis in which the intersection matrix is equivalent to $\bs{C}_\text{LT}$ is obtained by replacing differential forms with poles that are only regulated by the $\rho$ with an appropriate $\delta$-form.
That means, the limit taken in this way implies the following limit for the dual cohomology basis  $[\frac{dz}{z-x}+\frac{dz}{1-z}]_c\rightarrow \delta_x(z)$. 
%We neglect the part with a pole at $u=1$ on the dual side since it all contributions to the intersections from this term vanish after taking the limit $\rho=0$. \\
%To find a combination period matrices that belong to those intersections, we have to find appropriate rotations of the intersection matrices $C_\text{orders}/H_\text{orders}$ to those of $C_\text{LT}/H_\text{LT}$. Additionally, have the freedom to fix one more parameter, namely the period matrix. 
%Assume, in leading order, we want to obtain the Rieman bilinears for the period matrix defined in (\ref{pmatrel}).
As described above, we can also obtain the matrices of (\ref{leadingterm}) by taking appropriate rotations of the intersection matrices of (\ref{355}) and then taking the limit $\rho\rightarrow 0$. \fpnote{We can still improve this!} To this end, we define the transformation matrices
\begin{align}
\label{traf}
    \bs{T}_1&=\begin{pmatrix} 
1&0 \\ 0 & \rho   e^{-2\pi i \alpha_1 } 
    \end{pmatrix}\\
    \label{t2}
    \bs{T}_2&=\begin{pmatrix} 
1&0 \\ 0 & e^{2 i \pi  \alpha_1 \epsilon }
    \end{pmatrix}\\
    \label{t3}
     \bs{T}_3&=\begin{pmatrix} 
1&0 \\ 0 &\rho^{-1} 
    \end{pmatrix}\, . 
\end{align}
Then we obtain 
\begin{align}
    \left(\bs{C} \bs{T}_3^T\right)|_{\rho=0} = \bs{C}_{\text{LT}} \text{ and } \left(\bs{T}_1^T\bs{H}\bs{T}_2^T\right)|_{|\rho=0} =\bs{H}_{\text{LT}}\, . 
\end{align}
\csnote{Ich schaue mir morgen nochmal an woher dieses $e^{...}$ genau kommt und ob man das vll noch wegbekommt}
We apply these rotations also to the period matrix and its dual, obtaining: 
\begin{align}
    \left(\bs{T}_1\bs{P}\right)|_{\rho=0} = \bs{P}_{\text{rel}} \text{ and }\left(\bs{T}_3^T \bs{\check{P}} \bs{T}_2\right)|_{\rho=0} = \bs{\check{P}}_{\text{rel}}\, . 
\end{align}
%This is done by introducing the rotation
%\begin{align} 
%\label{traf}
%    \tilde{\bs{P}}= \bs{T} (\varepsilon)\bs{P} \text{ with %} \bs{T}(\varepsilon)=\begin{pmatrix} 
%1&0 \\ 0 & \alpha_x \varepsilon e^{-2\pi i %\alpha_1\varepsilon} 
%    \end{pmatrix}
%\end{align}
%that amounts to a change of the homology basis by
%\begin{align}
%\label{tildeH}
%  \tilde{\bs{H}}=\bs{T}(\varepsilon)^T \bs{H}  . 
%\end{align}
%The expansion of the period matrix takes the form 
%\begin{align}
%    \tilde{\bs{P}} = \bs{P}_\text{rel} +\mathcal{O}%(\rho)\, ,
%\end{align}
%where $\bs{P}_\text{rel}$ is the period matrix in (\ref{pmatrel}). 
%Further, we introduce the rotations 
%\begin{align}
 % \bs{\mathcal{H}}&=\bs{T}(\varepsilon)^T \bs{H} \bs{T}_2(\varepsilon)^T  \text{ with } \bs{T}_2(\varepsilon)=\begin{pmatrix} 
%-1&0 \\ 0 & -\frac{2 i \exp(i \pi  \varepsilon  (\alpha_{01}+2 \alpha_1)) \sin (\pi  \alpha_x \varepsilon ) \sin (\pi  \varepsilon  (\alpha_{01x}))}{\rho \pi(-1 + \exp(2 i \pi  \varepsilon \alpha_{01}))}
%    \end{pmatrix}\,,\\
%      \bs{\mathcal{C}}&= \bs{C} \bs{T}_3(\varepsilon)^T  \text{ with } \bs{T}_3(\varepsilon)=\begin{pmatrix} 
%1&0 \\ 0 &\rho^{-1} 
%    \end{pmatrix}\,.
%\end{align}
%Those rotations lead to 
%\begin{align}
%\bs{\mathcal{C}}|_{\rho=0}&=\bs{C}_\text{LT} \,, \quad \bs{\mathcal{H}}|_{\rho=0}=\bs{H}_\text{LT}
%\end{align}
%and corresponds to a rotation of the dual period matrix
%\begin{align}
%    \check{\bs{\mathcal{P}}}=\bs{T}^T_3(\varepsilon)\check{\bs{P}}\bs{T}_2(\varepsilon)\,.
%\end{align}
%We find that 
%\begin{align}
%    %\check{\bs{\mathcal{P}}}|_{\rho=0}=\check{\bs{P}}_\text{rel%}\,,
%\end{align}
%where $\check{\bs{P}}_\text{rel}$ is the dual period matrix obtained in the relative calculation in (\ref{pmatreldual}).\\\\
\noindent \textbf{Limit from the non-relative case, whilst preserving $\bs{\check{P}}=\bs{P}|_{\varepsilon\rightarrow -\varepsilon}$} To preserve the relation between the period matrix and its dual, we apply the transformation (\ref{traf}) \fpnote{Why is this transformation necessary for the limit?}\fpnote{We still need to remove the $\varepsilon$ here.} \csnote{ dachte das hatten wir letztens so abgesprochen, man kann die auch lassen und die homology von anfang an anders definieren aber hatten doch gesagt dass wir uns nicht ganz sicher sind ob zb A*[0,1] mit einem vorfaktor A richtig ist zu schreiben udn wir das deswegen als rotation machne}also to the dual period matrix so that
\begin{align}
   \check{\tilde{\bs{P}}}= \tilde{\bs{P}}(-\epsilon) = \bs{P}_\text{rel}(-\epsilon)+\mathcal{O}(\rho)\, . 
\end{align}
If we fix the dual period matrix like this, we cannot apply the other transformations so that for the intersection matrices,\fpnote{I don't understand this sentence.} these expansions take the form 
\begin{align}
 \tilde{\bs{H}} &=\begin{pmatrix}
     -\frac{i}{2} \left(\cot(\pi \alpha_0\varepsilon) +\cot(\pi \alpha_1\varepsilon)\right)&0\\ 0 & 0 
 \end{pmatrix}+\mathcal{O}(\rho) \,,\\
 \bs{C}^{-1} &= \begin{pmatrix}
-\epsilon&0\\ 0 & 0
 \end{pmatrix}+\mathcal{O}(\rho) \, . 
\end{align}
Note, that the leading order terms of both of these matrices are degenerate and hence not invertible, i.e. in the limit they are not associated to a complete basis of forms and contours. This means, that whilst we do obtain a dual period matrix that is related to the period matrix by $\varepsilon\rightarrow -\varepsilon$, this dual period matrix cannot be obtained from full bases of the dual (co-)homology groups in the target space. Consequently, we only obtain one quadratic relation in the limit, which is
\begin{align}
  -\frac{1}{2} i (\cot (\pi \alpha_0 \epsilon )+\cot (\pi \alpha_1 \epsilon ))=\frac{i \alpha_0  \alpha_{01}\epsilon \Gamma (-\alpha_0 \epsilon ) \Gamma (\alpha_0 \epsilon ) \Gamma (1-\alpha_1 \epsilon ) \Gamma (\alpha_1 \epsilon +1)}{2 \pi \alpha_1\Gamma (-\alpha_{01} \epsilon +1) \Gamma (\alpha_{01} \epsilon +1)}\, . 
\end{align}
\end{example}

To summarize, we have observed -- in agreement with \cite{Brunello:2023fef} --  that circumventing the relative framework via a regulator brings us to the same results as the relative framework, including the fact, that the dual period matrix cannot be chosen to be the $\varepsilon\rightarrow -\varepsilon$ limit of the period matrix. If we take the limit in such a way that this property is preserved, we obtain degenerate intersection matrices. In the former case, we obtain the same Riemann bilinear relations as in the relative framework, in the latter a subset of them. The only relation between the dual and non-dual period matrix is generally given by the Riemann bilinears. We have the freedom to either fix both period matrices and compute the corresponding intersection matrices (which might lead to a degenerate intersection matrix if the period matrices do not correspond to valid period matrices in the relative limit) or fix valid intersection parings, but have no control over one of the period matrices.
\csnote{glaube den ganzen absatz kann man noch kürzen}
\fpnote{Ich finde das eigentlich ganz gut. ich glaube aber wir könnten das alles zusammen fassen und vielleicht auch Beispiel und den absatz vorher direkt verbinden, weil das sowieso nicht sehr allgemein ist. oder ads vorher sehr kurz halten und alles ins beispiel rein. sollten wir heute nachmitag mal reeden. }

%\fpnote{
%\subsection*{To Do}
%\begin{itemize}
%\item Introduce (very shortly) twisted cohomology (refer to %much literature) 
%\item Introduce very shortly relative twisted cohomology (refer %to much literature) 
%\item Take as a running example the function $F_{21}$. 
%\item Already mention here, that in the twist we will only need %exponents $\varepsilon$ and $\frac{1}{2}+\varepsilon$
%\item Introduce Riemann bilinear relations 
%\item Make this very applicable to next sections. 
%\end{itemize}
%}



==> acknow.tex <==
We thank Andrzej Pokraka, Mathiue Giroux and Oliver Schlotterer for helpful discussions. This work [FP,CD] was co-funded by the European Union (ERC Consolidator Grant LoCoMotive 101043686). Views and opinions expressed are those of the author(s) only and do not necessarily reflect those of the European Union or the European Research Council. Neither the European Union nor the granting authority can be held responsible for them. 

==> sec_UneqSunrise_old.tex <==
% !TEX root = main.tex

As a first example, we consider the unequal-mass sunrise integral family in $D=2-2\varepsilon$ dimensions:
\begin{align}
\label{sunexstart}
I_{\bs{\nu}}^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];
                             \draw (-4pt,0) -- (4pt,0);}}}
\left(p^2,m_1^2,m_2^2,m_3^2 \right)= e^{2\gamma_E \varepsilon} \int \frac{\rd^D \ell_1}{i\pi^{D/2}} \frac{\rd^D \ell_2}{i\pi^{D/2}}\frac{1}{D_1^{\nu_1}D_2^{\nu_2}D_3^{\nu_3}}\, ,
\end{align}
with 
\beq\bsp
    D_1&\,=\ell_1^2-m_1^2\,,\\
     D_2&\,=(\ell_2-\ell_1)^2-m_2^2\,,\\
D_3&\,=(p+\ell_2)^2-m_3\, . 
\esp\eeq
%Computing the maximal cut of $I_{111}^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];
%                             \draw (-4pt,0) -- (4pt,0);}}}$ in the
Quadratic relations satisfied by the maximal cuts of the equal-mass sunrise have been investigated in ref.~\cite{Lee:2018jsw}. We now argue that these quadratic relations can be extended to the unequal-mass case. One of the main differences is that, in the unequal-mass case there are four master integrals for the maximal cuts, while there are only two in the equal-mass case.



                             Using the
loop-by-loop approach, we obtain the Baikov polynomial in one internal variable $z$, and we define the twist 
\begin{align}
    \Phi_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];
                             \draw (-4pt,0) -- (4pt,0);}}} =
z^\varepsilon \left[(z-\lambda_1)(z-\lambda_2)
(z-\lambda_3)(z-\lambda_4)\right]^{
-\frac{1}{2}-\varepsilon}\, ,
\end{align}
where
\beq\bsp
 \lambda_1&\,=-(m_1-m_2)^2\,,\\
 \lambda_2&\,=-(m_1+m_2)^2\,,\\
 \lambda_3&\,=-(m_3-p)^2\,,\\
  \lambda_4&\,=-(m_3+p)^2\, .
\esp\eeq
This twist defines a twisted cohomology group $H_{\text{dR}}^n (X, \nabla_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}})$ on the $X=\mathbb{C}-\{0,\lambda_1,\lambda_2,\lambda_3,\lambda_4
\}$. Note that in the limit $\varepsilon\rightarrow 0$, the Baikov polynomial reduces to the polynomial defining the elliptic curve attach to the sunrise integral, defined as the locus in $\mathbb{C}^2$ defined by
\begin{align}\label{curvesunrise}
y^2=p_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}}(z)= (z-\lambda_1)(z-\lambda_2)(z-\lambda_3)(z-\lambda_4)\, . 
\end{align}

Let us now discuss our choice of master integrals, or equivalent our choice of basis for $H_{\text{dR}}^n (X, \nabla_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}})$. A possible choice would be a logarithmic basis (and its regularised version), which leads a particularly simple intersection matrix.  %Taking the elliptic curve as a hyperelliptic function of genus 1 a possible 
However, our basis choice is inspired from a geometrical viewpoint for the elliptic curve defined by eq.~\eqref{curvesunrise}, where the standard basis consists of Abelian differentials of the first, third and second kind. This will allows us to easily obtain analytic expressions for some of the maximal cuts in terms of complete elliptic integrals of first and second kind.
%cf. ref \cite{Broedel_2018}. 
Explicitly, we choose the following basis for $H_{\text{dR}}^n (X, \nabla_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}})$:
\beq\bsp
\label{basissun}
\varphi_1^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,=\rd z
\,,\\
 \varphi_2^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,=\left(z^2 - \frac{s_1}{2} z + \frac{s_2}{6}\right)\rd z\,,\\
   \varphi_3^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,=
z \,\rd z\,,\\
\varphi_4^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,=\frac{\rd z}{z}\,,
\esp\eeq
We pick a basis of dual co-cycles according to eq.~\eqref{eq:FI_dual_basis}:
%To maintain the relation $\check{P}=P(-\varepsilon)$, the basis of the dual cohomology group $H_{\text{dR}}^n (X, \check{\nabla}_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}})$ is (the regularised version of)
\begin{align}
\check{\varphi}_i^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=\left[\frac{\varphi_i^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}}{p_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}}(z)}\right]_c
\,,\qquad i=1,\ldots,4\,.
%\check{\varphi}_2^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=\frac{\rd \varphi_2}{y_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}}},\,  \check{\varphi}_3^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=
%\frac{\varphi_3}{y_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}}}
%\text{ and }
%\check{\varphi}_4^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=\frac{\varphi_4}{y_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}}}
\end{align}
%Note that introducing the factor $y_{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt]; \draw (-4pt,0) -- (4pt,0);}}$ is equivalent to computing the intersection matrix between the cohomology basis (\ref{basissun}) and its regularised version as well as calculating an appropriate dimension shift matrix, as introduced in section \ref{quadrelmaxcut}. \fpnote{This sentence should be clearer.} 

Next, let us discuss our choice of maximal cut contours, or equivalently our choice of basis for the twisted homology group and its dual.
For the dual homology basis we choose cycles supported on
\beq\bsp
\label{dualbas}
    \check{\gamma}_1^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,=[\lambda_1,\lambda_2] \,,\\ 
    \check{\gamma}_2^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,=[\lambda_2,\lambda_3]  \,,\\ 
    \check{\gamma}_3^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,= [\lambda_1,\lambda_2]+[\lambda_3,\lambda_4]\,,\\
    \check{\gamma}_4^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}&\,= [\lambda_4,0]\, . 
\esp\eeq
This basis is depicted in figure~\ref{fig.cyclesell}, together with the canonical cycles $a$ and $b$ of the elliptic curve defined by eq.~\eqref{curvesunrise}. The basis of the twisted homology group is then supported on the regularised version of the dual cycles (cf.~eq.~\eqref{eq:check_to_h}):
\beq
\gamma_i^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}} = \big[\check{\gamma}_i^{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}\big]_{\textrm{reg}}\,,\qquad i =1\,\ldots,4\,.
\eeq

\begin{figure}[!t]
    \centering
    \includegraphics[align=c, scale=.4]{figuregenus1.pdf}
 \caption{%\claudecomment{We should remove the text that appears as inlay to the figure. Explanations about the figure should be in the caption, not as an inlay.}
 Our choice of (dual) twisted cycles is inspired by the geometric picture for the elliptic curve defined by eq.~\eqref{curvesunrise} has the two basis cycles $a$ and $b$, which inspire our choice of the dual twisted cycles $\check{\gamma}_1$ and $\check{\gamma}_2$. In the $\varepsilon \rightarrow 0$ limit, the cycle $\check{\gamma}_3$ corresponds to the cycle around infinity, so that if $\varphi_i$ has vanishing residue at infinity, and the period matrix simplifies. For generic $\varepsilon$ the twist has an additional factor $z^\varepsilon$ which requires us to add the dual twisted cycle $\check{\gamma}_4$.}
    \label{fig.cyclesell}
\end{figure}

With these choices for the bases of the (co-)homology groups and their duals, we obtain the following expressions for the intersection matrices (with $\bx = (p^2,m_1^2,m_2^2,m_3^2)$):
\begin{align} \label{csun}
\bC_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,\eps)&= \left(
\begin{array}{cccc}
 0 & \frac{1}{-3 \varepsilon -1} & 0 & 0 \\
 \frac{1}{1-3 \varepsilon } & -\frac{\varepsilon  (\lambda_2+\lambda_2+\lambda_3+\lambda_4)^2}{12 \left(9 \varepsilon ^2-1\right)} & \frac{\lambda_1+\lambda_2+\lambda_3+\lambda_4}{6-18 \varepsilon } & 0 \\
 0 & -\frac{\lambda_1+\lambda_2+\lambda_3+\lambda_4}{18 \varepsilon +6} & -\frac{1}{3 \varepsilon } & 0 \\
 0 & 0 & 0 & -\frac{1}{\lambda_1 \lambda_2 \lambda_3 \lambda_4 \varepsilon } \\
\end{array}
\right)\,,\\
\bH_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\eps)&=\left(
\begin{array}{cccc}
 i \tan (\pi  \varepsilon ) & -1+\frac{1}{1+e^{2 i \pi  \varepsilon }} & i \tan (\pi  \varepsilon ) & 0 \\
 \frac{1}{1+e^{2 i \pi  \varepsilon }} & i \tan (\pi  \varepsilon ) & -i \tan (\pi  \varepsilon ) & 0 \\
 i \tan (\pi  \varepsilon ) & -i \tan (\pi  \varepsilon ) & 2 i \tan (\pi  \varepsilon ) & -1+\frac{1}{1+e^{2 i \pi  \varepsilon }} \\
 0 & 0 & \frac{1}{1+e^{2 i \pi  \varepsilon }} & i \csc (2 \pi  \varepsilon ) \\
\end{array}
\right)\,.
\end{align}
The period matrix $\bP_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,\eps)$ can be expressed in terms of Lauricella functions, 
\beq\bsp
    F_D^{(n)} (a,b_1,\ldots,&b_n;c;x_1,\ldots,x_n) =\\
    =&\, \frac{\Gamma(c)}{\Gamma(a)\Gamma(c-a)} \int_0^1 \rd t\, t^{a-1} (1-t)^{c-a-1}\prod_{i=1}^n(1-x_it)^{-b_i},
\esp\eeq
valid for $\mathrm{Re}(c)>\mathrm{Re}(a)>0$,
and the dual period matrix is given by 
\beq
\check{\bP}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,\eps) = \bP_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,-\eps)\,.
\eeq

The TRBRs then take the form:
\beq\label{eq:sunrise_trbr}
\bP_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,\eps)^T\bC_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,\eps)\bP_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\bx,-\eps) = \bH_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\eps)\,.
\eeq
We have check numerically at various points that eq.~\eqref{eq:sunrise_trbr} holds. Since the entries of the period matrix are multi-valued functions, care is needed when evaluating the period matrix. 
We fix the branch for $\lambda_1<\lambda_2<\lambda_3<\lambda_4<0$. We note that the integral defining $P_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}},44}(\bx,\eps)$ is only defined for $\varepsilon>0$, while $\check{P}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}},44}(\bx,\eps)$ is defined for $\varepsilon <0$, due to the occurrence of a non-integrable singularity at $z=0$ otherwise. But in the TRBRs, we have to evaluate the expressions at a single value for $\varepsilon$. In order to circumvent this issue, we have performed a carefull analytic continuation of the Lauricella function to the entire complex plane. 

It is interesting to investigate what eq.~\eqref{eq:sunrise_trbr}. Indeed, we expect that in limit $\eps\to0$, four entries in the period matrix reduce to the periods and quasi-period of the elliptic curve defined by eq.~\eqref{curvesunrise}. The latter are related by the well-known Legendre relation between elliptic integrals of the first and second kind, 
\begin{align}
  \K(1-\lambda) \E(\lambda)+ \E(1-\lambda)-\K(\lambda)\K(1-\lambda)=\frac{\pi}{2}\,,
\end{align}
with 
\beq
\K(\lambda) = \int_{0}^1\frac{\rd t}{\sqrt{(1-t^2)(1-\lambda t^2)}}\qquad \textrm{~~and~~}
\E(\lambda) = \int_{0}^1\rd t\,\sqrt{ \frac{1-\lambda t^2}{1-t^2}}\,.
\eeq
Since our period matrix is a $4\times4$, it is interesting to see how the Legendre relation is recovered, and if there are any new relations that go beyond it. We start by expanding eq.~\eqref{eq:sunrise-trbr} in $\eps$, and we observe that $H_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}},44}(\eps) = \mathcal{O}\left({\varepsilon^{-1}}\right)$. In order to obtain a finite limit, we introduce an additional rotation of the homology basis:
\begin{align}
    \bT_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\varepsilon)=\left(
\begin{array}{cccc}
 1& 0& 0& 0 \\
0 & 1 & 0 & 0 \\
 0 & 0 &1 & 0 \\
 0 & 0 &0 & \varepsilon \\
\end{array}
\right)\,,
\end{align}
to define $\tilde{P}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=P_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}T_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\varepsilon)$ and $\tilde{H}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=T_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\varepsilon)H_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}T_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(-\varepsilon)$. In leading order, we obtain from $  \tilde{P}^{(0),T}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}\left(C^{-1,T}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}\right)^{(0)}\tilde{P}^{(0)}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}=\tilde{H}^{(0)}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}$ the relations
\begin{align}
 \left(
\begin{array}{cccc}
 0 & \frac{i (\xi_2 \omega_1-\xi_1 \omega_2)}{2 \pi } & 0 & 0 \\
 \frac{i (\xi_1 \omega_2-\xi_2 \omega_1)}{2 \pi } & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 \\
\end{array}
\right)+\mathcal{O}(\varepsilon)=\left(
\begin{array}{cccc}
 0 & -\frac{1}{2} & 0 & 0 \\
\frac{1}{2} & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 \\
 0 & 0 & 0 & 0 \\
\end{array}
\right)+\mathcal{O}(\varepsilon)\,.
\end{align}
The periods of $\tilde{P}^{(0)}_{{\tikz[baseline=-0.5ex]{\draw (0,0) circle [radius=2pt];\draw (-4pt,0) -- (4pt,0);}}}(\varepsilon)$ are given by 
\begin{align}
    \omega_1&=\frac{1}{c_4} K(\lambda)\,,\quad \omega_2=\frac{i}{c_4}K(1-\lambda)\\
    \xi_1&=-2 c_4 \left(E(\lambda)-\frac{2-\lambda}{3}K(\lambda)\right)\,, \quad \xi_2=-2 c_4 \left(-iE(1-\lambda)-i \frac{1+\lambda}{3}K(1-\lambda)\right)\,,
\end{align}
\sfsnote{is there a reason for the $c_4$ prefactors?}
with $\lambda=\frac{(\lambda_1-\lambda_4) (\lambda_2-\lambda_3)}{(\lambda_1-\lambda_3) (\lambda_2-\lambda_4)}$
and $c_4=\frac{1}{2} \sqrt{(\lambda_1-\lambda_3) (\lambda_2-\lambda_4)}$. The only non-trivial relations we obtain can be rewritten as 
\begin{align}
  K(1-\lambda) E(\lambda)+K(\lambda) (E(1-\lambda)-K(1-\lambda))=\frac{\pi}{2}\,,
\end{align}
which are the well-known Legendre relations.

